The State of Computer Vision Research in Africa

Despite significant efforts to democratize artificial intelligence (AI), computer vision which is a sub-field of AI, still lags in Africa. A significant factor to this, is the limited access to computing resources, datasets, and collaborations. As a result, Africa's contribution to top-tier publications in this field has only been 0.06% over the past decade. Towards improving the computer vision field and making it more accessible and inclusive, this study analyzes 63,000 Scopus-indexed computer vision publications from Africa. We utilize large language models to automatically parse their abstracts, to identify and categorize topics and datasets. This resulted in listing more than 100 African datasets. Our objective is to provide a comprehensive taxonomy of dataset categories to facilitate better understanding and utilization of these resources. We also analyze collaboration trends of researchers within and outside the continent. Additionally, we conduct a large-scale questionnaire among African computer vision researchers to identify the structural barriers they believe require urgent attention. In conclusion, our study offers a comprehensive overview of the current state of computer vision research in Africa, to empower marginalized communities to participate in the design and development of computer vision systems.

==> content/author_def.tex <==
%
% --- inline annotations
%
\usepackage{colortbl}

% % user-specific edits: 
\newcommand{\luk}[1]{{\color{darkcyan} #1}} % Lukman
\newcommand{\men}[1]{{\color{red} #1}} % Menna
\newcommand{\ash}[1]{{\color{green} #1}} % Ashery
\newcommand{\dan}[1]{{\color{purple} #1}}
\newcommand{\userE}[1]{{\color{cyan} #1}}
\newcommand{\userH}[1]{{\color{olive} #1}}
\newcommand{\userI}[1]{{\color{violet} #1}}
\newcommand{\userJ}[1]{{\color{maroon} #1}}
\newcommand{\userK}[1]{{\color{navy} #1}}

% comment section above and uncomment the section below for final submission (changes all text to black)

% \newcommand{\luk}[1]{{#1}}
% \newcommand{\men}[1]{{#1}}
% \newcommand{\ash}[1]{{#1}}
% \newcommand{\dan}[1]{{#1}}
% \newcommand{\userE}[1]{{#1}}
% \newcommand{\userF}[1]{{#1}}
% \newcommand{\userG}[1]{{#1}}
% \newcommand{\userH}[1]{{#1}}
% \newcommand{\userI}[1]{{#1}}
% \newcommand{\userJ}[1]{{#1}}



==> content/results2.tex <==
\subsection{Summary and Discussion}
In this section, we summarize our results and list open questions. Our analysis has shown that African researchers are key contributors to African research, yet there exist multiple barriers facing Africans across all regions to publish in top-tier venues. We showed African contributions constituting only 0.06\% over the last ten years. It brings the question of, \textbf{what could be these potential barriers and how to improve our research eco-system to overcome them?} It also showed the current trend of topics published in Africa, bringing the question of whether our research is addressing our most urgent needs. \textbf{Is \emph{Image Encryption} the most needed topic in Central or Northern Africa?} Moreover, it showed the current gap in the Central Africa region concerning other regions, and the dominance of the Northern region in computer vision publications. It still showed a recent increase in research output from Eastern and Western Africa. Nonetheless, it brings the question of \textbf{how to increase the computer vision research capacity in Africa and especially Central Africa?} 

In order to discuss the first open question within a participatory framework, we ask 14 community members from Egypt, Nigeria, Cameroon and Benin about the barriers facing African computer vision research, suggestions to improve it and its strengths. We ensure to take their informed consent. Note, that this is a discussion to incorporate our own stories in the work to lead the way to a large-scale quantitative study for our future work. The responses from the community members showed a wide agreement that some of the main barriers in Africa~\citep{de2018machine} include, lack of funding, limited availability of data, poor economic systems and low access to resources. Another barrier is the existence of peer-reviewing bias in venues as previously documented~\citep{tomkins2017reviewer}. Additionally, the responses showed that there can be a disconnect between academic research and industry, which might be attributed to lack of well established datasets collected from the continent, and lack of incentives for companies and startups to conduct research. Another barrier is the unreasonable teaching loads on the graduate students and low compensation for academics and researchers. Low incentives from institutions to conduct high quality research. There is also lack of in-depth technical knowledge in computer vision in Africa when compared to general machine learning. Moreover, the low quality of education in some of the African institutions makes the students struggle. Finally, the low presence of senior researchers or academics who can provide mentorship and supervision is also a contributing barrier, since African researchers tend to travel outside Africa. Some of the strengths in the African countries, as a general consensus from the community, is the presence of many computer vision problems (e.g. healthcare, education, etc.) that are specifically relevant to Africa. These diverse problems open the door for significant contributions from African researchers. Moreover, the abundance of passionate African researchers that want to help their communities. Accordingly, there is a need for funding, collaborations between academia and industry, access to training and resources to engage these passionate researchers in their communities' needs. 
 



\subsection{A Discussion on the structural barriers in Africa}
summarize points from above and insights + relate to the structural barriers and discuss the survey that will conducted on the type of structural barriers that caused this discrepancy int he results + identify strength points as well and what we can do to improve.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\todo{Note: Review for modification}

In this section we report the results of the refined set manual validation, then we describe the results of our three analysis types: (i) a geo-temporal analysis where we study different African regions' publishing patterns over the last ten years, (ii) a collaboration patterns analysis, and (iii) a keywords analysis. Throughout all the analysis we follow~\citep{african_regions} in defining the five African regions. We choose to conduct a fine-grained study per region instead of comparing Northern \textit{vs.} sub-Saharan Africa, in order to assess the equity in computer vision research within the continent itself.

\subsection{Manual validation results}

We start with verifying the results  of our \emph{refined} set, in terms of the topic, that it belongs to computer vision, and the authors, that they include at least one African author. We randomly select 5\% of the refined set of publications, that were manually verified by the team. Each paper was assigned two annotators. For the topic verification, we manually inspected the abstract, as for the authors we ensured at least one African institution existed in the affiliations. Our results for the topic verification show 91.1\% accuracy with only 8.9\% of the publications wrongly assigned as computer vision. In the authors verification, we report 98.4\% accuracy, where it demonstrates that most of our errors were from irrelevant topics rather than the authors. Moreover, we report high inter-annotator agreement of 93.9\% and 96.7\% in both the topic and the authors verification, resp.

\subsection{Geo-temporal analysis}
\label{sec:geotemporal_analysis}

We start with demonstrating the publishing patterns for the different African regions in the computer vision field over the last ten years (2012-2022). Figure~\ref{fig:geotemporal_refined} (A, B) shows the number of publications and percentages resp., on the logarithmic scale, from the \emph{refined} set with at least one author working in an African institution. Publications with authors affiliated with institutions from two different African countries are accounted for in each country and region, as we are studying the computer vision research capacity. Figure~\ref{fig:geotemporal_refined} (A) shows that institutions in Northern and Southern Africa are the two highest regions publishing in computer vision. They construct around 88.5\% of the total publications in the \emph{refined} set over the last ten years, and exhibit consistent growth over the years. 

\input{graphs/refined_african_pubs}

Looking upon Eastern and Western Africa we notice growth of the publications over the period 2016-2022. Interestingly, Figure~\ref{fig:geotemporal_refined} (B) shows that the percentage of publications originating from Eastern and Western regions combined has grown from 5.1\% in 2016 to 19.9\% in 2022, closing the gap with Southern Africa. Nonetheless, the gap between sub-Saharan and Northern African remains. More importantly, when looking to Central Africa it is the most in need of building capacity for computer vision research, contributing only 0.9\% of the total publications.
%\input{graphs/full_african_pubs}

The \emph{refined} set has one fifth of the publications in the \emph{full} set, but has gone through a verification process making it more accurate, as explained in Section~\ref{sec:method}. Nonetheless, we contrast the geo-temporal analysis for both the \emph{refined} and \emph{full} sets, where we show in Figure~\ref{fig:geotemporal_refined} (C) the number of publications in the \emph{full} set for the different African regions over the last ten years. It still shows that the Northern and Southern regions are the highest two regions publishing, with around 85\% from the total of publications stemming from them. It also has Central Africa the least region publishing in computer vision and only contributing around 0.85\%. Thus, it aligns with our previous \emph{refined} set findings.

The previous analysis shows some of the strength points of the computer vision research in Africa such as the development of Western and Eastern African regions to have a better capacity in computer vision research from 2016 till 2022. Moreover, the growth trends in both Northern and Southern regions computer vision publications show promising potential. Yet, our main weakness is the wide gap between the Northern region \textit{vs.} the rest of Africa, especially Central Africa which needs investment in improving their computer vision research. 

Additionally, we analyze the top ten African countries publishing in computer vision. Figure~\ref{fig:top10} (Left) shows the annual publications for each of the top ten African countries publishing in computer vision, and Figure~\ref{fig:top10} (right) lists these top ten countries with their total publications over the last ten years. They show growth over the years in their number of publications, yet most of them belong to the Northern and Southern regions. Positively, it demonstrates that a country like Ethiopia, outside these two regions, went from zero publications in 2012-2013 to 148 publications in 2022. 

\input{graphs/top5_countries}

%\input{graphs/top10institutions}
%Figure Test~\ref{fig:top10instituions}
To assess the equity in computer vision research and access of African researchers to opportunities and publishing in top-tier venues, we perform a separate geo-temporal analysis on these publications only. We mainly focus on the toughest and highest ranking computer vision conferences (i.e., \emph{CVPR, ICCV and ECCV}), the best machine learning conferences that do accept computer vision publications (i.e., \emph{ICML, NeurIPS and ICLR}), the top medical image processing conference (i.e., \emph{MICCAI}) and the top computer vision journals (i.e., \emph{TPAMI} and \emph{IJCV}). Figure~\ref{fig:toptier} shows the number of publications in the aforementioned venues across the different continents over the last ten years. We show the publication-researcher pairs as we want to fairly document the number of researchers from African institutions that can publish in these leading venues. It clearly shows that North America and Asia are the ones mostly publishing in top-tier venues with around three quarters (74\%) of these publications stemming from them. Moreover, they show a consistent increase in publications over the years, especially Asia which surpassed North America in the last two years. However, when looking to Africa it only constitutes 0.06\% of the total publications, and over the years it does not show a consistent increase and growth in the number of publications. Interestingly, we found that Madagascar had two researchers that published in \emph{ICLR} 2022, which shows the promise of how a small under-resourced country was still able to publish in a leading venue as such. Nonetheless, when we compare Africa in general to South America which is another under-resourced continent, we see that South America has more publications where it constitutes around 0.23\% of the total \emph{top-tier} set. This confirms that Africans do not have the same opportunities and access to conduct such research with respect to other continents even when compared to ones that are low resourced. It brings the question of why and what can be done to improve the situation in Africa.

We conduct a similar study but with focus on \emph{Computer Vision and Pattern Recognition (CVPR)} conference only as the well established and frequent venue in computer vision. Additionally, we highlight the African authors affiliated with non African institutions using their affiliation history as a proxy. We identified 49 authors that were affiliated with non African institutions but had an African institution in their affiliation history. Figure~\ref{fig:toptier_cvonly} shows both African authors in African institutions (red) and African authors even if affiliated with non African institutions (blue). It shows worse trends, where Africa constitutes only 0.02\% of the total \emph{CVPR} publications over the last ten years and in certain years no publications (i.e., 2012-2013, 2018-2021). It confirms on the problem as these results are recent, and showing that these issues still persist. It motivates our pursue of first documenting the problem then starting a discussion on why this is the case. However, when we look at the African authors not necessarily affiliated with African institutions, we see a promising potential where their publications constitute 0.2\% of the last ten year \emph{CVPR} publications. This most likely stems from international institutions admitting African graduate students and welcoming them to increase diversity within research and encourage these researchers to pursue their career. Yet, it still begs the question of why the same researchers did not publish in \emph{CVPR} at their African institutions, what can be done to bridge this gap.

\input{graphs/toptier_geotemporal}
\input{graphs/toptier_cvonly_geotemporal}

\subsection{Collaboration patterns analysis}
\input{graphs/collabs_africavsintern}

In order to understand the collaboration patterns in African computer vision publications, we conduct two types of analysis on the \emph{refined} set. First we analyze the African \textit{vs.} international collaborations in terms of the number of publications over the last ten years. Figure~\ref{fig:collabs_africa_vs_international} (A) demonstrates that most of the publications are dominated by international collaborations with very minimal amount of African collaborations~\citep{pouris2014research,turki2023machine}, forming only 3.9\% of the total publications. Since African countries share some of the problems and bottlenecks they are facing, pan-African collaborations can strengthen the continent's research eco-system. Moreover, it can result in a better focus on our own problems, and will make the reciprocal engagements between the affected communities and researchers easier as the researchers belong to these affected communities. Nonetheless, we think that international collaborations does improve African research in other aspects, because of the fact that the continent is limited in resources (e.g. compute). These collaborations can help overcome these barriers. Hence, why we believe that a balance between pan-African and international collaborations is necessary towards an independent African computer vision research eco-system. We also list here the top ten countries outside Africa that act as international collaborators: France (28\%), Saudi Arabia (16.6\%), United States (14.3\%), India (8.8\%), China (8.2\%), United Kingdom (7.9\%), Canada (5.3\%), Germany (4.7\%), Spain (3.8\%), and United Arab Emirates(2.4\%). We list the countries with the percentages of publications for each. %with respect to the total publications output in collaboration with Africa.

Second, we analyze the role of African authors in such publications, whether they are a key-contributor (i.e., first or last author) or rather a co-author that is not a key contributor. In this analysis publications that have same African country with differing roles (e.g., first and last) are counted twice in each role. Figure~\ref{fig:collabs_africa_vs_international} (B) shows the amount of publications per year with first, last African authors or others. It clearly shows a good strength point in our community, where most of the publications have African authors as key contributors in the work either as first or last authors.

\subsection{Keywords analysis}
\input{graphs/keywork_regional}
% \input{graphs/keyword_reg}
% 
In our final analysis, we study the research topics and recurring keywords in the computer vision field in Africa on the \emph{full} set of publications. In this analysis we choose to do it using the \emph{full} instead of the \emph{refined} set, since the \emph{refined} set depends on the top 50 keywords from global computer vision in their query generation. Thus, it can skew the results. These keywords are retrieved using an off-the-shelf tool as described in Section~\ref{sec:method_details}. Out of 187,812 keywords we only identify the top-30 recurring ones. In Figure~\ref{fig:plot_highly_cited} (A-E), we show these top-30 keywords per African region, to identify which one is the mostly researched per region. We also show in Figure~\ref{fig:plot_highly_cited} (F) the co-occurrence matrix between pairs of these keywords, which can be used to understand certain keywords that non experts in the topic might not be aware of. For example, \emph{Hyperchaotic Systems} is highly co-occurring with \emph{Image Encryption}, where we see that it does relate to techniques in cryptography. %Other examples include \emph{Hyperspectral Imagery}/\emph{Remote Sensing} and \emph{Steganography/Image Encryption}.
Surprisingly, we found keywords such as \emph{Galaxies} and \emph{Crystalline Texture}, to verify their relevance we inspect five random publications for each. We found that \emph{Crystalline Texture} is used in publications related to texture classification which is relevant to computer vision. However, the keyword \emph{Galaxies} is used in publications that are relevant~\citep{fielding2022classification}, but others are not~\citep{shirley2021help}.



Inspecting the top-30 keywords distribution per African region in Figure~\ref{fig:plot_highly_cited} (A), it shows that Northern Africa has \emph{Image Segmentation}, \emph{Object Detection} as the most recurring keywords. Interestingly, Figure~\ref{fig:plot_highly_cited} (B) shows the most recurring keyword in Southern Africa is \emph{Galaxies}, which is hard to discern automatically whether it is relevant to computer vision or not as detailed earlier. The next common keywords are \emph{Animals}, \emph{Crops} and keywords related to \emph{Remote Sensing} (e.g., \emph{Landsat}). Figure~\ref{fig:plot_highly_cited} (C, D) show both Eastern and Western Africa with the most common keywords \emph{Landsat} and \emph{Land Cover}. Figure~\ref{fig:plot_highly_cited} (E) shows the most common keywords in Central Africa is related to \emph{Image Encryption}. The question of whether certain regions are working on the most urgent needs or not, remains unanswered but it is beyond the scope of this study.
%. Although, answering such a question is beyond this study but documenting the current state of computer vision research in Africa is the first step.
%\begin{itemize}
%\item a visualization of topic clusters and topic names overall
%\item Analysis per African region on the topics of interest
%\end{itemize}




==> graphs/collabs_order.tex <==
\begin{figure}
\centering

\caption{Collaborations pattern analysis showing the distribution of African authors as a key contributor to the project (i.e. first/last authors) \textit{vs} contributing as co-authors.}
\label{fig:authors_order}
\end{figure}

==> graphs/keyword_reg.tex <==
\pgfplotstableread{ % data 
Label	FALSE	TRUE
Steganography	11.4	88.6
{Crystalline Texture}	12.1	87.9
{Computer Vision}	33.2	66.8
Crops	59.5	40.5
Landsat	62.3	37.7
Videorecording	14.8	85.2
{Hyperspectral Imagery}	19	81
Nanocrystal	34.3	65.7
{Radiological Findings}	21	79
{Clinical Features}	21	79
Animals	49.5	50.5
Mammography	23.1	76.9
{Breast Neoplasms}	25.9	74.1
Galaxies	97.1	2.9
Camera	24.7	75.3
Biometry	20.6	79.4
{Land Cover}	62.9	37.1
{Image Segmentation}	8.9	91.1
COVID-19	25.9	74.1
{Hyperchaotic System}	14.3	85.7
Cryptography	12.3	87.7
{Image Encryption}	11.6	88.4
{Convolutional Neural Network}	20.3	79.7
{Remote Sensing}	49.5	50.5
Cancer	24	76
{Case Report}	25.8	74.2
{Magnetic Resonance Imaging}	22.2	77.8
IOU	28.3	71.7
{Object Detection}	27.6	72.4
{Deep Learning}	27.9	72.1
}\testdataN

\pgfplotstableread{ % data 
Label	FALSE	TRUE
Steganography	97.7	2.3
{Crystalline Texture}	94.5	5.5
{Computer Vision}	81.3	18.7
Crops	67.6	32.4
Landsat	73.8	26.2
Videorecording	92.7	7.3
{Hyperspectral Imagery}	87.8	12.2
Nanocrystal	71.2	28.8
{Radiological Findings}	92.5	7.5
{Clinical Features}	92.5	7.5
Animals	68.1	31.9
Mammography	92.8	7.2
{Breast Neoplasms}	88.9	11.1
Galaxies	5.1	94.9
Camera	85.9	14.1
Biometry	88.3	11.7
{Land Cover}	75.5	24.5
{Image Segmentation}	96.1	3.9
COVID-19	89.1	10.9
{Hyperchaotic System}	98.7	1.3
Cryptography	98.9	1.1
{Image Encryption}	98.7	1.3
{Convolutional Neural Network}	91.9	8.1
{Remote Sensing}	77.4	22.6
Cancer	88.2	11.8
{Case Report}	90	10
{Magnetic Resonance Imaging}	87.2	12.8
IOU	87.3	12.7
{Object Detection}	87.5	12.5
{Deep Learning}	87.2	12.8
}\testdataS

\pgfplotstableread{ % data  
Label	FALSE	TRUE
Steganography	95.3	4.7
{Crystalline Texture}	97.5	2.5
{Computer Vision}	90.1	9.9
Crops	82.2	17.8
Landsat	79.8	20.2
Videorecording	96.9	3.1
{Hyperspectral Imagery}	95.7	4.3
Nanocrystal	95.2	4.8
{Radiological Findings}	95	5
{Clinical Features}	95	5
Animals	90.6	9.4
Mammography	92.6	7.4
{Breast Neoplasms}	92.6	7.4
Galaxies	97.1	2.9
Camera	95.5	4.5
Biometry	97.9	2.1
{Land Cover}	79.6	20.4
{Image Segmentation}	97.1	2.9
COVID-19	93.5	6.5
{Hyperchaotic System}	97.8	2.2
Cryptography	98.5	1.5
{Image Encryption}	98.5	1.5
{Convolutional Neural Network}	93.9	6.1
{Remote Sensing}	86.2	13.8
Cancer	92.6	7.4
{Case Report}	92.5	7.5
{Magnetic Resonance Imaging}	96	4
IOU	92.1	7.9
{Object Detection}	92.2	7.8
{Deep Learning}	92.7	7.3
}\testdataE

\pgfplotstableread{ % data  
Label	FALSE	TRUE
Steganography	95.3	4.7
{Crystalline Texture}	95.9	4.1
{Computer Vision}	94.2	5.8
Crops	86.5	13.5
Landsat	81.2	18.8
Videorecording	95.6	4.4
{Hyperspectral Imagery}	97.2	2.8
Nanocrystal	93.4	6.6
{Radiological Findings}	89.2	10.8
{Clinical Features}	89.2	10.8
Animals	91.6	8.4
Mammography	89.1	10.9
{Breast Neoplasms}	91.5	8.5
Galaxies	98.7	1.3
Camera	95.1	4.9
Biometry	91.6	8.4
{Land Cover}	80	20
{Image Segmentation}	97.6	2.4
COVID-19	88.8	11.2
{Hyperchaotic System}	96.8	3.2
Cryptography	96.4	3.6
{Image Encryption}	97.1	2.9
{Convolutional Neural Network}	93	7
{Remote Sensing}	85.1	14.9
Cancer	92.8	7.2
{Case Report}	91.5	8.5
{Magnetic Resonance Imaging}	94.1	5.9
IOU	91.3	8.7
{Object Detection}	91.7	8.3
{Deep Learning}	91.1	8.9 
}\testdataW

\pgfplotstableread{ % data 
Label	FALSE	TRUE
Steganography	99.7	0.3
{Crystalline Texture}	99.7	0.3
{Computer Vision}	99.5	0.5
Crops	98.9	1.1
Landsat	94.5	5.5
Videorecording	99.7	0.3
{Hyperspectral Imagery}	99.5	0.5
Nanocrystal	99.7	0.3
{Radiological Findings}	98.5	1.5
{Clinical Features}	98.5	1.5
Animals	97.5	2.5
Mammography	99.3	0.7
{Breast Neoplasms}	100	0.0
Galaxies	100	0.0
Camera	98	2
Biometry	99.8	0.2
{Land Cover}	94.1	5.9
{Image Segmentation}	99.8	0.2
COVID-19	98.3	1.7
{Hyperchaotic System}	89.9	10.1
Cryptography	91.9	8.1
{Image Encryption}	92.1	7.9
{Convolutional Neural Network}	99.4	0.6
{Remote Sensing}	96	4
Cancer	99.2	0.8
{Case Report}	98.7	1.3
{Magnetic Resonance Imaging}	99.2	0.8
IOU	99.3	0.7
{Object Detection}	99.4	0.6
{Deep Learning}	99.3	0.7
}\testdataC

\pgfplotstableread{ % data 
Label              Number
{IOU/Deep Learning}                             16.62002677
{Object Detection/Deep Learning}                16.62002677
{Object Detection/IOU}                          16.62002677
{Hyperchaotic System/Cryptography}               6.959484122
{Image Encryption/Hyperchaotic System}           6.959484122
{Image Encryption/Cryptography}                  6.959484122
{Clinical Features/COVID-19}                     4.866772113
{Radiological Findings/COVID-19}                 4.866772113
{Radiological Findings/Clinical Features}        4.866772113
{Remote Sensing/Landsat}                         4.161090157
{Remote Sensing/Land Cover}                      4.112422436
{Landsat/Land Cover}                             4.015086994
{Remote Sensing/Hyperspectral Imagery}            1.070689865
{Mammography/Breast Neoplasms}                    0.6691811656
{Deep Learning/Convolutional Neural Network}      0.1825039543
{Videorecording/Steganography}                    0.1581700937
{Steganography/Image Encryption}                  0.09733544227
{Cancer/Breast Neoplasms}                         0.09733544227
{Image Segmentation/Hyperspectral Imagery}        0.04866772113
{Computer Vision/Camera}                           0.03650079085
}\Coocurrence
% \begin{figure}[!ht]
% \centering
% \resizebox{0.5\textwidth}{!}{



 
\begin{figure}[H]
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \resizebox{0.9\linewidth}{!}{
            \begin{tikzpicture}
                 \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataN}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={ at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(A) Northern Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataN};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataN};    
                    \legend{False, True}
                \end{axis}
            \end{tikzpicture}
        }
         
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
    \centering
        \resizebox{0.9\linewidth}{!}{
            \begin{tikzpicture}
               \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataS}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(B) Southern Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataS};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataS};    
                    \legend{False, True}
                \end{axis}
            \end{tikzpicture}
        }
         
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \resizebox{0.9\linewidth}{!}{
            \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataE}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(C) Eastern Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataE};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataE};    
                    \legend{False, True}
                \end{axis}
            \end{tikzpicture}
        } 
         
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \resizebox{0.9\linewidth}{!}{
        \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataW}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(D) Western Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataW};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataW};    
                    \legend{False, True}
                \end{axis}
        \end{tikzpicture}
    } 
     
    \end{subfigure}
        \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \resizebox{0.9\linewidth}{!}{
        \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataC}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(E) Central Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataC};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataC};    
                    \legend{False, True}
                \end{axis}
        \end{tikzpicture}
    } 
     
\end{subfigure}%
        \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \resizebox{0.9\linewidth}{!}{
        \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=20,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\Coocurrence}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.2)},anchor=north, below=5mm},
                    xlabel = {(F) Co-occurrence Matrix},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=Number, meta=Label,y expr=\coordindex] {\Coocurrence};   % "First" column against the data index
                    %\addplot table [x=Most-cited, meta=Label,y expr=\coordindex] {\testdataC};    
                    %\legend{True, False}
                \end{axis}
        \end{tikzpicture}
    } 
     
\end{subfigure}
\caption{Keywords analysis of the top-30 keywords. (A-E) Distribution of the most recurring keywords per African region. Red indicates the percentage of publications within the corresponding region indexed with that keyword. (F) The top co-occurrent keywords.}
\label{fig:plot_highly_cited}
\end{figure}

 

==> graphs/keyword_regional.tex <==

\pgfplotstableread{ % data 
Label	FALSE	TRUE
Steganography	11.4	88.6
{Crystalline Texture}	12.1	87.9
{Computer Vision}	33.2	66.8
Crops	59.5	40.5
Landsat	62.3	37.7
Videorecording	14.8	85.2
{Hyperspectral Imagery}	19	81
Nanocrystal	34.3	65.7
{Radiological Findings}	21	79
{Clinical Features}	21	79
Animals	49.5	50.5
Mammography	23.1	76.9
{Breast Neoplasms}	25.9	74.1
Galaxies	97.1	2.9
Camera	24.7	75.3
Biometry	20.6	79.4
{Land Cover}	62.9	37.1
{Image Segmentation}	8.9	91.1
COVID-19	25.9	74.1
{Hyperchaotic System}	14.3	85.7
Cryptography	12.3	87.7
{Image Encryption}	11.6	88.4
{Convolutional Neural Network}	20.3	79.7
{Remote Sensing}	49.5	50.5
Cancer	24	76
{Case Report}	25.8	74.2
{Magnetic Resonance Imaging}	22.2	77.8
IOU	28.3	71.7
{Object Detection}	27.6	72.4
{Deep Learning}	27.9	72.1
}\testdataN

\pgfplotstableread{ % data 
Label	FALSE	TRUE
Steganography	97.7	2.3
{Crystalline Texture}	94.5	5.5
{Computer Vision}	81.3	18.7
Crops	67.6	32.4
Landsat	73.8	26.2
Videorecording	92.7	7.3
{Hyperspectral Imagery}	87.8	12.2
Nanocrystal	71.2	28.8
{Radiological Findings}	92.5	7.5
{Clinical Features}	92.5	7.5
Animals	68.1	31.9
Mammography	92.8	7.2
{Breast Neoplasms}	88.9	11.1
Galaxies	5.1	94.9
Camera	85.9	14.1
Biometry	88.3	11.7
{Land Cover}	75.5	24.5
{Image Segmentation}	96.1	3.9
COVID-19	89.1	10.9
{Hyperchaotic System}	98.7	1.3
Cryptography	98.9	1.1
{Image Encryption}	98.7	1.3
{Convolutional Neural Network}	91.9	8.1
{Remote Sensing}	77.4	22.6
Cancer	88.2	11.8
{Case Report}	90	10
{Magnetic Resonance Imaging}	87.2	12.8
IOU	87.3	12.7
{Object Detection}	87.5	12.5
{Deep Learning}	87.2	12.8
}\testdataS

\pgfplotstableread{ % data  
Label	FALSE	TRUE
Steganography	95.3	4.7
{Crystalline Texture}	97.5	2.5
{Computer Vision}	90.1	9.9
Crops	82.2	17.8
Landsat	79.8	20.2
Videorecording	96.9	3.1
{Hyperspectral Imagery}	95.7	4.3
Nanocrystal	95.2	4.8
{Radiological Findings}	95	5
{Clinical Features}	95	5
Animals	90.6	9.4
Mammography	92.6	7.4
{Breast Neoplasms}	92.6	7.4
Galaxies	97.1	2.9
Camera	95.5	4.5
Biometry	97.9	2.1
{Land Cover}	79.6	20.4
{Image Segmentation}	97.1	2.9
COVID-19	93.5	6.5
{Hyperchaotic System}	97.8	2.2
Cryptography	98.5	1.5
{Image Encryption}	98.5	1.5
{Convolutional Neural Network}	93.9	6.1
{Remote Sensing}	86.2	13.8
Cancer	92.6	7.4
{Case Report}	92.5	7.5
{Magnetic Resonance Imaging}	96	4
IOU	92.1	7.9
{Object Detection}	92.2	7.8
{Deep Learning}	92.7	7.3
}\testdataE

\pgfplotstableread{ % data  
Label	FALSE	TRUE
Steganography	95.3	4.7
{Crystalline Texture}	95.9	4.1
{Computer Vision}	94.2	5.8
Crops	86.5	13.5
Landsat	81.2	18.8
Videorecording	95.6	4.4
{Hyperspectral Imagery}	97.2	2.8
Nanocrystal	93.4	6.6
{Radiological Findings}	89.2	10.8
{Clinical Features}	89.2	10.8
Animals	91.6	8.4
Mammography	89.1	10.9
{Breast Neoplasms}	91.5	8.5
Galaxies	98.7	1.3
Camera	95.1	4.9
Biometry	91.6	8.4
{Land Cover}	80	20
{Image Segmentation}	97.6	2.4
COVID-19	88.8	11.2
{Hyperchaotic System}	96.8	3.2
Cryptography	96.4	3.6
{Image Encryption}	97.1	2.9
{Convolutional Neural Network}	93	7
{Remote Sensing}	85.1	14.9
Cancer	92.8	7.2
{Case Report}	91.5	8.5
{Magnetic Resonance Imaging}	94.1	5.9
IOU	91.3	8.7
{Object Detection}	91.7	8.3
{Deep Learning}	91.1	8.9 
}\testdataW

\pgfplotstableread{ % data 
Label	FALSE	TRUE
Steganography	99.7	0.3
{Crystalline Texture}	99.7	0.3
{Computer Vision}	99.5	0.5
Crops	98.9	1.1
Landsat	94.5	5.5
Videorecording	99.7	0.3
{Hyperspectral Imagery}	99.5	0.5
Nanocrystal	99.7	0.3
{Radiological Findings}	98.5	1.5
{Clinical Features}	98.5	1.5
Animals	97.5	2.5
Mammography	99.3	0.7
{Breast Neoplasms}	100	0.0
Galaxies	100	0.0
Camera	98	2
Biometry	99.8	0.2
{Land Cover}	94.1	5.9
{Image Segmentation}	99.8	0.2
COVID-19	98.3	1.7
{Hyperchaotic System}	89.9	10.1
Cryptography	91.9	8.1
{Image Encryption}	92.1	7.9
{Convolutional Neural Network}	99.4	0.6
{Remote Sensing}	96	4
Cancer	99.2	0.8
{Case Report}	98.7	1.3
{Magnetic Resonance Imaging}	99.2	0.8
IOU	99.3	0.7
{Object Detection}	99.4	0.6
{Deep Learning}	99.3	0.7
}\testdataC

\pgfplotstableread{ % data 
Label              Number
{IOU/Deep Learning}                             16.62002677
{Object Detection/Deep Learning}                16.62002677
{Object Detection/IOU}                          16.62002677
{Hyperchaotic System/Cryptography}               6.959484122
{Image Encryption/Hyperchaotic System}           6.959484122
{Image Encryption/Cryptography}                  6.959484122
{Clinical Features/COVID-19}                     4.866772113
{Radiological Findings/COVID-19}                 4.866772113
{Radiological Findings/Clinical Features}        4.866772113
{Remote Sensing/Landsat}                         4.161090157
{Remote Sensing/Land Cover}                      4.112422436
{Landsat/Land Cover}                             4.015086994
{Remote Sensing/Hyperspectral Imagery}            1.070689865
{Mammography/Breast Neoplasms}                    0.6691811656
{Deep Learning/Convolutional Neural Network}      0.1825039543
{Videorecording/Steganography}                    0.1581700937
{Steganography/Image Encryption}                  0.09733544227
{Cancer/Breast Neoplasms}                         0.09733544227
{Image Segmentation/Hyperspectral Imagery}        0.04866772113
{Computer Vision/Camera}                           0.03650079085
}\Coocurrence

\begin{figure*}[!ht]
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \resizebox{1\linewidth}{!}{
            \begin{tikzpicture}
                 \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataN}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={ at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(A) Northern Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataN};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataN};    
                    \legend{False, True}
                \end{axis}
            \end{tikzpicture}}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\linewidth}
    \centering
        \resizebox{1\linewidth}{!}{
            \begin{tikzpicture}
               \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataS}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(B) Southern Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataS};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataS};    
                    \legend{False, True}
                \end{axis}
            \end{tikzpicture}}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \resizebox{1\linewidth}{!}{
            \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataE}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(C) Eastern Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataE};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataE};    
                    \legend{False, True}
                \end{axis}
            \end{tikzpicture}} 
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataW}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(D) Western Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataW};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataW};    
                    \legend{False, True}
                \end{axis}
        \end{tikzpicture}} 
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=100,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\testdataC}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.23)},anchor=north, below=5mm},
                    xlabel = {(E) Central Africa},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=FALSE, meta=Label,y expr=\coordindex] {\testdataC};   % "First" column against the data index
                    \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\testdataC};    
                    \legend{False, True}
                \end{axis}
        \end{tikzpicture}} 
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tikzpicture}
                \begin{axis}[
                    xbar stacked,   % Stacked horizontal bars
                    bar width = 4pt,
                    xmin=0,         % Start x axis at 0
                    xmax=20,
                    ytick=data,     % Use as many tick labels as y coordinates
                    legend style={at={(0.5, 1.05)}, anchor=north, legend columns=-1},
                    yticklabels from table={\Coocurrence}{Label},  % Get the labels from the Label column of the \datatable
                    x label style={at={(0.5, 1.2)},anchor=north, below=5mm},
                    xlabel = {(F) Co-occurrence Matrix},
                    % enlarge x limits = {value = .1},
                    % enlarge y limits={abs=4pt}
                    y tick label style={font=\tiny}
                    ]
                    \addplot table [x=Number, meta=Label,y expr=\coordindex] {\Coocurrence};   % "First" column against the data index
                    % \addplot table [x=TRUE, meta=Label,y expr=\coordindex] {\Coocurrence};    
                    
                \end{axis}
        \end{tikzpicture} } 
\end{subfigure}

\caption{Keywords analysis of the top-30 keywords. (A-E) Distribution of the most recurring keywords per African region. Red indicates the percentage of publications within the corresponding region indexed with that keyword. (F) The top co-occurrent keywords. \textcolor{red}{We need to redesign that plot to save space maximum half page but still see the keywords}}
\label{fig:plot_highly_cited}
\end{figure*}

 

==> graphs/table_authors.tex <==
\begin{table}[h!]
\centering
\caption {African Authors. \textcolor{red}{To save space can we move that table to the github repository}}
\begin{tabular}{ c @{\hskip 0.7in} c }
\hline
Author Name & Country\\
\hline
 Mkhinini Maher  & Tunisia\\ 
 Warrell Jonathan & South Africa\\  
 Malti Abed & Algeria\\
 Elhabian Shireen Y. & Egypt\\
 Farag Aly A. & Egypt\\
 Elgammal Ahmed & Egypt\\
 Badri Hicham & Morocco\\
 Laga Hamid & Algeria\\
 Abdelrahim Aly S. & Egypt\\
 Elhoseiny Mohamed & Egypt\\
 Hefeeda Mohamed & Egypt\\
 Abdelrahman Mostafa & Egypt\\
 Belbachir Ahmed Nabil & Algeria\\
 Ibrahim Mostafa S. & Egypt\\
 Kamel Abdelrahman & Egypt\\
 Haouchine Nazim & Algeria\\
 Drira Hassen & Tunisia\\
 Abdelhamed Abdelrahman & Egypt\\
 Fathy Mahmood & Egypt\\
 Bargal Sarah Adel & Egypt\\
 Joty Shafiq  & Egypt\\
 Afifi Mahmoud & Egypt\\
 Meshry Moustafa & Egypt\\
 Aly Mohamed Sabry & Egypt\\
 Benzine Abdallah & Algeria\\
 Eldesokey Abdelrahman & Egypt\\
 Bourahla Omar & Algeria\\
 Ouali Yassine & Morocco\\
 Abdelaziz Ibrahim & Egypt\\
 Chehata N. & Tunisia\\
 Sabry Aly Mohamed M. & Egypt\\
 Taha Ahmed & Egypt\\
 Snoussi Hichem & Tunisia\\
 Ward Rabab & Egypt \\
Elkerdawy Sara & Egypt \\
Elhoushi Mostafa & Egypt \\
Metwaly Kareem & Egypt \\
Kahla Mostafa & Egypt \\
Siam Mennatullah & Egypt \\
Boujemaa Nozha & Tunisia \\
Mkhinini Maher & Tunisia \\
Baji Ivan V. & South Africa \\
Otberdout Naima & Morocco \\
Daoudi Mohamed & Morocco \\
Markham Andrew & South Africa \\
Amayo Paul & South Africa\\
Li Jonathan & South Africa \\
Burke Michael & South Africa \\
Hancke Gerhard P. & South Africa \\
\hline
\end{tabular}
\end{table}

==> tables/datasets_official.tex <==
% % Dataset and other related tables
% % Dataset and other related tables

% %######################################################################
%  % Official Dataset
% %######################################################################

% % 


% \begin{table*}[h!]
% \centering
% {\fontsize{7}{9}\selectfont 

% \caption{Officially Published African Datasets \textcolor{red}{Agriculture related -> Forest/Agriculture related - Forest,Agriculture related->Forest/Agriculture related - Animals, Wildlife related-> Animals/Wildlife related - Please update all categories some are old, fix centering problem of the whole table same in other table}
% \ash{Updated}} 
% \label{tab:official_dataset}
% \begin{tabular}{|c|l|l|c|c|l|} 
% \hhline{|======|}
%    & \textbf{Category}             & \textbf{Dataset Name}    & \textbf{Publicly Available}       & \textbf{Year} & \textbf{Venue}            \\ 
% \hhline{|======|}
% %1  & \begin{tabular}[c]{@{}l@{}}Image Classification,\\Animals, Wildlife related\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}DSAIL-Porini~\cite{mugambi2023dsail}\end{tabular}                                                 &             & 2023          & \begin{tabular}[c]{@{}l@{}}Data in Brief\end{tabular}           \\ 
% %\hline
% 1  & \begin{tabular}[c]{@{}l@{}}Video: Action and Event Understanding, \\Humans: Face, Body, Pose, Gesture, Movement\end{tabular}             
% & \begin{tabular}[c]{@{}l@{}}Ego4D Dataset~\cite{grauman2022ego4d}\end{tabular}                       & \checkmark\footnotemark{\url{https://ego4d-data.org}}           & 2022          
% & \begin{tabular}[c]{@{}l@{}}CVPR\end{tabular}                     \\ 
% \hline
% 2  & \begin{tabular}[c]{@{}l@{}}Object Detection,\\ Waste Detection\end{tabular}               
% & \begin{tabular}[c]{@{}l@{}}ZeroWaste Dataset~\cite{bashkirova2022zerowaste}\end{tabular}                                                       &       \checkmark\footnotemark{\url{http://ai.bu.edu/zerowaste/}}                                                                                                                            & 2022          & CVPR                                                                                                                                            \\ 
% \hline
% 3 & \begin{tabular}[c]{@{}l@{}}Multi-modal Learning, \\Image Captioning\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Hausa Visual Genome~\cite{abdulmumin2022hausa}\end{tabular}                                                                                                                                        &    \checkmark\footnotemark{\url{ http://hdl.handle.net/11234/1-4749}}                                                                                                                               & 2022          & \begin{tabular}[c]{@{}l@{}}ACL\end{tabular}                                                      \\ 
% \hline
% 4  & \begin{tabular}[c]{@{}l@{}}Medical and Biological Vision,\\Image Classification\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}Predicting COVID-19~\cite{muhammad2022deep}\end{tabular}                                                                                    &   \checkmark\footnotemark{\url{https://drive.google.com/file/d/\\1bum9Sehb3AzUMHLhBMuow\\PKyr\_PCrB3a/view}}                                                                                                                                & 2022          & \begin{tabular}[c]{@{}l@{}}Trends and Advancements \\of Image Processing \\and Its Applications\end{tabular}                                                   \\ 
% \hline
% %6  & \begin{tabular}[c]{@{}l@{}}Object Detection,\\Object Recognition\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}Egyptian Licence Plates\cite{youssef2022new}\end{tabular}                                                                                      &                                                                                                                                   & 2022          & \begin{tabular}[c]{@{}l@{}}ACIRS\end{tabular}                                                   \\ 
% %\hline
% 5  & \begin{tabular}[c]{@{}l@{}}Agriculture related, \\Image Segmentation\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Avo-AirDB~\cite{amraoui2022avo}\end{tabular}                  &                                                                                \checkmark\footnotemark{\url{https://data.mendeley.com\\/datasets/tvhh83r3hj/2}}                                                   & 2022          & \begin{tabular}[c]{@{}l@{}}Data in Brief\end{tabular}                                                             \\ 
% \hline
% 6 & \begin{tabular}[c]{@{}l@{}}Photogrammetry and \\Remote Sensing,\\Image Segmentation\end{tabular}           & \begin{tabular}[c]{@{}l@{}}Land cover map of Vavatenina region\\ (Madagascar)~\cite{lelong2022land}\end{tabular}                                                                                                                         &   \checkmark\footnotemark{\url{https://doi.org/10.18167/DVN1/XJCXCS}}\footnotemark{\url{https://doi.org/10.18167/DVN1/KDNOV4}}               & 2022          & \begin{tabular}[c]{@{}l@{}}Data in Brief\end{tabular}                                                                           \\ 
% \hline
% 7 & \begin{tabular}[c]{@{}l@{}}Document Analysis and Understanding,\\Object Recognition\end{tabular}               & \begin{tabular}[c]{@{}l@{}}Scanned Arabic Books~\cite{elanwar2021extracting}\end{tabular}                                                          &      \checkmark\footnotemark{\url{https://github.com/wdqin/BE-Arabic-9K}}           & 2021          & IJDAR         \\ 
% \hline
% %10 & \begin{tabular}[c]{@{}l@{}}Photogrammetry and Remote\\Sensing, Agriculture Related\end{tabular}               & \begin{tabular}[c]{@{}l@{}}Assessing soil cover levels using multitemporal \\satellite imagery~\cite{laamrani2020assessing}\end{tabular}                                                          &                                                                                                                                   & 2020          & Remote Sensing                                                                                                                                            \\ 
% %\hline
% 8  & \begin{tabular}[c]{@{}l@{}}Medical and Biological Vision, \\ Object Detection \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Malaria and Sickle Cells Detection\\ in Blood Films~\cite{manescu2020weakly}\end{tabular} &  \checkmark\footnotemark{\url{https://doi.org/10.5522/04/12407567}}  &     2020          & \begin{tabular}[c]{@{}l@{}}MICCAI\end{tabular}\\
% \hline
% 9 & \begin{tabular}[c]{@{}l@{}}Climate related, \\Video: Action and Event Understanding\end{tabular}           & \begin{tabular}[c]{@{}l@{}}Photographed Lightning Events\\ South Africa~\cite{hunt2020dataset}\end{tabular} &     \checkmark\footnotemark{\url{ http://dx.doi.org/10.17632/44vkdvrn67.1}}       & 2020          & Data in Brief                                                                                                                                        \\ 
% \hline
% 10  & \begin{tabular}[c]{@{}l@{}}Animals/Wildlife related \\Photogrammetry and Remote Sensing,\end{tabular} & \begin{tabular}[c]{@{}l@{}}Effects of Land cover change on Great Apes\\ distribution in South East Cameroon~\cite{yuh2019effects}\end{tabular}                                                                                                                  & Request\footnotemark{\url{http://apes.eva.mpg.de/}}    & 2019          & \begin{tabular}[c]{@{}l@{}}Scientific Reports\end{tabular}                                                                        \\ 
% \hline
% %14  & \begin{tabular}[c]{@{}l@{}}Photogrammetry and \\Remote Sensing, \\Agriculture Related\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Determination of the age of oil palm, the case of\\ Ejisu-Juaben district, Ghana~\cite{chemura2015determination}\end{tabular}                  &                                                                                                                                   & 2015          & \begin{tabular}[c]{@{}l@{}}ISPRS Journal of \\Photogrammetry\\and Remote Sensing\end{tabular}                                                             \\ 
% %\hline
% %15  & \begin{tabular}[c]{@{}l@{}}Image Segmentation\\Photogrammetry and Remote Sensing\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Mapping of Land Cover Changes\\ in Lake Hawassa~\cite{wondrade2014gis}\end{tabular}                                                                                                             &              & 2014          & \begin{tabular}[c]{@{}l@{}}Environmental Monitoring\\ and Assessment\end{tabular} \\ 
% %\hline
% \end{tabular} }
% \end{table*}

% \vcell{Weighted Correlation Matrix G2}   
% \vcell{\begin{tabular}[b]{@{}l@{}}Weighted \\Correlation Matrix G2\end{tabular}}

% \begin{table*}[ht]
\begin{sidewaystable*}[!htbp]
% \centering
{\fontsize{7}{9}\selectfont
\caption{Officially published datasets with at least one African institution.}
\label{tab:official_dataset}
\begin{tabular}{|c|l|l|c|l|}

\hhline{|=====|}
& \textbf{Category} & \textbf{Dataset Name} & \textbf{Available} & \textbf{Venue} \\
\hhline{|=====|}

1 & \makecell[l]{Video: Action and Event Understanding\\Humans: Face, Body, \\Pose, Gesture, Movement} & Ego4D Dataset~$(1)$ & \checkmark\footnotemark & CVPR \\
\hline
2 & \makecell[l]{Object Detection\\ Waste Detection} & ZeroWaste Dataset~$(2)$ & \checkmark\footnotemark & CVPR \\
\hline
3 & \makecell[l]{Multi-modal Learning \\Image Captioning } & Hausa Visual Genome~$(3)$ & \checkmark\footnotemark & LREC \\
\hline
4 & \makecell[l]{Medical and Biological Vision\\Image Classification} & Predicting COVID-19 $(4)$ & \checkmark\footnotemark & \makecell[l]{Trends and Advancements \\of Image Processing \\and Its Applications} \\
\hline
5 & \makecell[l]{Forests, Plants, Agriculture related\\ Image Segmentation} & Avo-AirDB $(5)$ &\checkmark\footnotemark & Data in Brief \\
\hline
6 & \makecell[l]{Photogrammetry and Remote Sensing\\Image Segmentation} & \makecell[l]{Land cover map of Vavatenina region\\ (Madagascar)~$(6)$ }& \checkmark\footnotemark\checkmark\footnotemark & Data in Brief\\
\hline
7 & \makecell[l]{Document Analysis and Understanding\\Image Classification} & Scanned Arabic Books~$(7)$ & \checkmark\footnotemark & IJDAR \\
\hline
8 & \makecell[l]{Medical and Biological Vision \\ Object Detection} & \makecell[l]{Malaria and Sickle Cells Detection\\ in Blood Films~$(8)$ }& \checkmark\footnotemark & MICCAI \\
\hline
9 & \makecell[l]{Climate related\\ Video: Action and Event Understanding} & \makecell[l]{Photographed Lightning Events\\ SA~$(9)$ } & \checkmark\footnotemark & Data in Brief \\
\hline
10 & \makecell[l]{Animals, Wildlife related \\Photogrammetry and Remote Sensing} & \makecell[l]{Effects of Land cover change on Great Apes \\ distribution in South East Cameroon~$(10)$ } & - & Scientific Reports \\
\hline

\end{tabular}
}
%\caption{Example table with checkmarks and footnotes}
\vspace{1em}
\tiny{
\\\\

$(1)$ \cite{grauman2022ego4d}\\
$(2)$ \cite{bashkirova2022zerowaste}\\
$(3)$ \cite{abdulmumin2022hausa}\\
$(4)$ \cite{muhammad2022deep}\\
$(5)$ \cite{amraoui2022avo} \\
$(6)$ \cite{lelong2022land}\\
$(7)$ \cite{elanwar2021extracting}\\
$(8)$ \cite{manescu2020weakly}\\
$(9)$ \cite{hunt2020dataset}\\
$(10)$ \cite{yuh2019effects} }
\end{sidewaystable*}


% \end{table*}


% Footnote texts
\addtocounter{footnote}{-10} % Adjust the counter to the number of footnotes
\stepcounter{footnote}\footnotetext{\url{https://ego4d-data.org}}
\stepcounter{footnote}\footnotetext{\url{http://ai.bu.edu/zerowaste/}}
\stepcounter{footnote}\footnotetext{\url{http://hdl.handle.net/11234/1-4749}}
\stepcounter{footnote}\footnotetext{\url{https://drive.google.com/file/d/1bum9Sehb3AzUMHLhBMuowPKyr\_PCrB3a/view}}
\stepcounter{footnote}\footnotetext{\url{https://data.mendeley.com/datasets/tvhh83r3hj/2}}
\stepcounter{footnote}\footnotetext{\url{https://doi.org/10.18167/DVN1/XJCXCS}}
\stepcounter{footnote}\footnotetext{\url{https://doi.org/10.18167/DVN1/KDNOV4}}
\stepcounter{footnote}\footnotetext{\url{https://github.com/wdqin/BE-Arabic-9K}}
\stepcounter{footnote}\footnotetext{\url{https://doi.org/10.5522/04/12407567}}
\stepcounter{footnote}\footnotetext{\url{http://dx.doi.org/10.17632/44vkdvrn67.1}}
%\stepcounter{footnote}\footnotetext{\url{http://apes.eva.mpg.de/}}

% ... more footnote texts ...

==> tables/datasets_unofficial.tex <==


% %\begin{center}
% \begin{table*}[h!]
% \centering
% {\fontsize{7}{10}\selectfont


% \caption{Non-official African Datasets.}
% \label{tab:nonofficial_dataset}

% \begin{tabular}{|c|l|l|l|l|c|} 
% \hhline{|======|}
%    & \textbf{Category}                                                                                                                             & \textbf{Dataset Name}                                                                                             & \textbf{Short Description}                                                                                                            & \textbf{Publicly Available}                                                                                                                                                           & \textbf{Country}                                                     \\ 
% \hhline{|======|}
% 1  & \begin{tabular}[c]{@{}l@{}}Image Classification, \\ Autonomous Driving \end{tabular}    
%    & MIIA Pothole  
%    & \begin{tabular}[c]{@{}l@{}}Images of South African streets with \\or without  potholes\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}
%        \checkmark\footnote{\url{https://zindi.africa/competitions/miia-poth\\ole-image-classification-challenge/data}}
%    \end{tabular}                                           
%    & \begin{tabular}[c]{@{}c@{}}South \\Africa\end{tabular}               \\ 
% \hline
% 2  & \begin{tabular}[c]{@{}l@{}} Food/Nutrition related, \\ Object Recognition\end{tabular}  
%    & Nigeria Food Ai Dataset 
%    & \begin{tabular}[c]{@{}l@{}}Images of 14 distinct \\indigenous Nigerian dishes\end{tabular}                         
%    & 
%    \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://www.kaggle.com/datasets/\\elinteerie/nigeria-food-ai-dataset/data}}
%    \end{tabular}                                                      
%    & Nigeria  \\ 
% \hline
% 3  & \begin{tabular}[c]{@{}l@{}}Agriculture related, \\Object Recognition \end{tabular}      
%    & Kenya Crop Type Detection 
%    & Images of crop fields.                                                                                             & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://www.kaggle.com/datasets/\\warcoder/kenya-crop-type-detection}}
%    \end{tabular}
%    & Kenya                                                                \\ 
% \hline
% 4  & \begin{tabular}[c]{@{}l@{}}Image Segmentation, \\ Humans: Face, Body, Pose, Gesture, Movement \end{tabular}       
%    & Spot the Mask Challenge 
%    & \begin{tabular}[c]{@{}l@{}}Images of people \\wearing masks.\end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://zindi.africa/competitions/\\spot-the-mask/data}}
%    \end{tabular}                                                                         
%    & -                                                                    \\ 
% \hline
% 5  & \begin{tabular}[c]{@{}l@{}}Image Segmentation, \\Image Classification\end{tabular}   
%    & Road Segment Identification 
%    & \begin{tabular}[c]{@{}l@{}}Images of different landscapes \\with or without road segments.\end{tabular}            & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://zindi.africa/competitions/\\road-segment-identification/data}}
%    \end{tabular}             
%    & \begin{tabular}[c]{@{}c@{}}South \\Africa\end{tabular}               \\ 
% \hline
% 6  & \begin{tabular}[c]{@{}l@{}}Animals/Wildlife related, \\ Object detection \\\end{tabular}                   
%    & \begin{tabular}[c]{@{}l@{}}Local Ocean Conservation\\~Sea Turtle Face Detection\end{tabular} 
%    & Images of sea turtles.                                                                                             & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://zindi.africa/competitions/\\local-ocean-conservation-sea\\-turtle-face-detection/data}}
%    \end{tabular}                                  
%    & Kenya                                                                \\ 
% \hline

% 7  & \begin{tabular}[c]{@{}l@{}}Object Recognition, \\Object Detection\end{tabular} 
%    & \begin{tabular}[c]{@{}l@{}}Bill Classification in\\Tunisia Challenge\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}Receipts images of restaurants, \\parking, fuel and transport\end{tabular}              & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://zindi.africa/competitions/\\bill-classification-in-tunisia-challenge/data}}\end{tabular}                                              
%    & Tunisia                                                              \\ 
% \hline
% 8  & \begin{tabular}[c]{@{}l@{}}Object Recognition, \\Object detection\end{tabular} 
%    & \begin{tabular}[c]{@{}l@{}}Computer Vision for License\\~Plate Recognition Challenge\end{tabular}                  & Vehicle images                                                                                                     & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://zindi.africa/competitions/ai-hack-\\tunisia-2-computer-vision-challenge-2/dat}}
%    \end{tabular}                                         
%    & Tunisia                                                              \\ 
% \hline
% 9  & \begin{tabular}[c]{@{}l@{}}Agriculture related, \\Object Detection\end{tabular} 
%    & \begin{tabular}[c]{@{}l@{}}Digital Africa Plantation \\Counting Challenge\end{tabular}                                   & Images contains palm trees                                                                                               & \begin{tabular}[c]{@{}l@{}}
%    \checkmark\tablefootnote{\url{https://zindi.africa/competitions/digital-\\africa-plantation-counting-challenge/data}}\end{tabular}                                          
%    & \begin{tabular}[c]{@{}c@{}}Cˆote \\d’Ivoire\end{tabular}             \\ 
% \hline
% 10  & \begin{tabular}[c]{@{}l@{}}Object Recognition, \\Humans: Face, Body, Pose, Gesture, Movement \\\end{tabular} 
%     & \begin{tabular}[c]{@{}l@{}}Task Mate Kenyan Sign\\Language Classification\\Challenge\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}Images contains Kenya\\Signs Languages.\end{tabular}                                   & \begin{tabular}[c]{@{}l@{}}
%     \checkmark\tablefootnote{\url{https://zindi.africa/competitions/\\kenyan-sign-language-classification\\-challenge/data}}
%     \end{tabular}                                       
%     & Kenya                                                                \\ 
% \hline
% \end{tabular} }

% \end{table*}
% %\end{center}





% \begin{table*}[ht]
\begin{sidewaystable*}[!htbp]
\centering
{\fontsize{7}{9}\selectfont 
\caption{Unofficial African Datasets.} 
\label{tab:nonofficial_dataset}
\begin{tabular}{|c|l|l|c|l|c|}
\hhline{|======|}
   & \textbf{Category}      & \textbf{Dataset Name}  & \textbf{Available}  & \textbf{Short Description}  & \textbf{Country}     \\ 
\hhline{|======|}

1  & \makecell[l]{Image Classification\\ Autonomous Driving, ADAS,\\ Transportation related}  & Pothole & \checkmark\footnotemark & \makecell[l]{Images of South African streets with \\or without  potholes} & \makecell{South \\Africa}  \\
\hline
2  & \makecell[l]{Food, Nutrition related\\ Image Classification} & Nigeria Food AI Dataset & \checkmark\footnotemark & \makecell[l]{Images of 14 distinct indigenous \\Nigerian dishes } & Nigeria  \\ 
\hline
3 & \makecell[l]{Forests, Plants, Agriculture related\\ Image Classification}  & Kenya Crop Type Detection &  \checkmark\footnotemark     & \makecell[l]{Images of crop fields}  &  Kenya  \\ 
\hline
4 & \makecell[l]{Image Segmentation\\ Humans: Face, Body, \\Pose, Gesture, Movement} & Spot the Mask Challenge  & \checkmark\footnotemark & \makecell[l]{Images of people wearing masks.} & - \\ 
\hline
5  &\makecell[l]{Image Segmentation \\Image Classification} & \makecell[l]{Road Segment Identification} &\checkmark\footnotemark  & \makecell[l]{Images of different landscapes \\with or without road segments} & \makecell[c]{South \\Africa }                                                          \\ 
\hline
6 & \makecell[l]{Animals, Wildlife related\\ Object Detection} & \makecell[l]{Local Ocean Conservation\\~Sea Turtle Face Detection} & \checkmark\footnotemark & Images of sea turtles. & Kenya \\                   
\hline
7 & \makecell[l]{Image Classification} & \makecell[l]{Bill Classification in\\Tunisia Challenge} & \checkmark\footnotemark & \makecell[l]{Images of receipts in restaurants, \\parking lots, and others} & Tunisia \\ 
\hline
8  & \makecell[l]{Image Classification\\ Object detection}  & \makecell[l]{Computer Vision for License\\~Plate Recognition Challenge}& \checkmark\footnotemark  & Images of vehicle licence plates  & Tunisia \\
\hline
9 & \makecell[l]{Forests, Plants, Agriculture related\\ Object Detection} & \makecell[l]{Digital Africa Plantation \\Counting Challenge} & \checkmark\footnotemark  & Images containing palm trees & \makecell[c]{C$\hat{o}$te\\d’Ivoire} \\ 
\hline
10  & \makecell[l]{Image Classification\\ Humans: Face, Body, \\Pose, Gesture, Movement} &\makecell[l]{Task Mate Kenyan Sign\\Language Classification\\Challenge} & \checkmark\footnotemark  & \makecell[l]{Images containing Kenyan\\sign language gestures} & Kenya \\ 
\hline
\end{tabular}}
%\caption{Example table with checkmarks and footnotes}

\end{sidewaystable*}
% \end{table*}


% Footnote texts
\addtocounter{footnote}{-10} % Adjust the counter to the number of footnotes
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/miia-pothole-image-classification-challenge/data}} %1
\stepcounter{footnote}\footnotetext{\url{https://www.kaggle.com/datasets/elinteerie/nigeria-food-ai-dataset/data}} %2
\stepcounter{footnote}\footnotetext{\url{https://www.kaggle.com/datasets/warcoder/kenya-crop-type-detection}} %3
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/spot-the-mask/data}} %4
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/road-segment-identification/data}}%5
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/local-ocean-conservation-sea-turtle-face-detection/data}}
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/bill-classification-in-tunisia-challenge/data}}
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/ai-hack-tunisia-2-computer-vision-challenge-2/dat}}
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/digital-africa-plantation-counting-challenge/data}}
\stepcounter{footnote}\footnotetext{\url{https://zindi.africa/competitions/kenyan-sign-language-classification-challenge/data}}

% ... more footnote texts ...
